Network Flow Models for Robust Binary Optimization with Selective Adaptability

Adaptive robust optimization problems have received significant attention in recent years, but remain notoriously difficult to solve when recourse decisions are discrete in nature. In this paper, we propose new reformulation techniques for adaptive robust binary optimization (ARBO) problems with objective uncertainty. Without loss of generality, we focus on ARBO problems with "selective adaptability", a term we coin to describe a common class of linking constraints between first-stage and second-stage solutions. Our main contribution revolves around a collection of exact and approximate network flow reformulations for the ARBO problem, which we develop by building upon ideas from the decision diagram literature. Our proposed models can generate feasible solutions, primal bounds and dual bounds, while their size and approximation quality can be precisely controlled through user-specified parameters. Furthermore, and in contrast with existing solution methods, these models are easy to implement and can be solved directly with standard off-the-shelf solvers. Through an extensive set of computational experiments, we show that our models can generate high-quality solutions and dual bounds in significantly less time than popular benchmark methods, often by orders of magnitude.

==> RCalgorithm.tex <==
\begin{algorithm}[h]
%\setstretch{1.15}
\caption{A row-and-column generation solution method}
\label{algo:RC}
\vspace{0.1cm}
%\textbf{Input:} An inverse MILO problem instance $(\bc^0, \hat\bx, \mX)$, initial trust region size $p^0$\\
%\textbf{Output:} An inverse-optimal solution $\bc^*$
\begin{algorithmic}[1]
%\State Initialization: $i=1$, $\tilde\mX^0 = \{ \hat\bx \}$.
\State Initialize $i=0, \, \Xi^0 = \{\xi^0\}$. 
\State Solve model \ref{model:main_BSO}, and obtain $v(\Xi^i)$ (lower bound) and $\bhy^i$. 
\State Call the oracle and obtain $v(\bhy^i)$ (upper bound) and $\xi^{i+1}$.
%\State If $v(\Xi^i) = v(\bhy^i)$, then we are done.
\State If $v(\Xi^i) < v(\bhy^i)$, set $\Xi^{i+1} = \Xi^{i} 
\cup \{\xi^{i+1}\}, i = i + 1$, return to Step 2.\\
\Return $v^* = v(\bhy^{i}), \ \bhy^* = \bhy^i$ %$\bc^* = \bhc^i$
\end{algorithmic}
\end{algorithm}

==> Tikz_Examples/Assignment_Ex.tex <==
\begin{figure}[h]
\centering
\begin{subfigure}[t]{0.45 \textwidth}
\centering
\resizebox{0.35\textwidth}{!}{
  \begin{tikzpicture}[-latex]
    \node[draw, circle, semithick, minimum size = 0.4cm] (i1) {$1$};
    \node[draw, circle, semithick, minimum size = 0.4cm] (i2) [below= 0.4cm of i1]  {$2$};
    \node[draw, circle, semithick, minimum size = 0.4cm] (i3) [below = 0.4cm of i2]  {$3$};
    \node[draw, circle, very thick, minimum size = 0.7cm] (j1) [right = 1.5cm of i1]  {a};
    \node[draw, circle, semithick, minimum size = 0.7cm] (j2) [below = 0.4cm of j1]  {b};
    \node[draw, circle, very thick, minimum size = 0.7cm] (j3) [below = 0.4cm of j2]  {c};
    \node[draw, circle, semithick, minimum size = 0.7cm] (j4) [below = 0.4cm of j3]  {d};
    %\node[draw, circle, fill = gray!15,minimum size = 0.15cm] (i4) [below = 0.4cm of i3]  {$i_4$};

    \path[draw, gray, line width = 0.05mm]
    (i1) edge node [xshift = -0.3cm] {} (j1)
    (i1) edge node [xshift = -0.3cm] {} (j2)
    (i1) edge node [xshift = -0.3cm] {} (j3)
    (i1) edge node [xshift = -0.3cm] {} (j4)
    (i2) edge node [xshift = -0.3cm] {} (j1)
    (i2) edge node [xshift = -0.3cm] {} (j2)
    (i2) edge node [xshift = -0.3cm] {} (j3)
    (i2) edge node [xshift = -0.3cm] {} (j4)
    (i3) edge node [xshift = -0.3cm] {} (j1)
    (i3) edge node [xshift = -0.3cm] {} (j2)
    (i3) edge node [xshift = -0.3cm] {} (j3)
    (i3) edge node [xshift = -0.3cm] {} (j4);
    %(i4) edge node [xshift = -0.3cm] {} (j1)
    %(i4) edge node [xshift = -0.3cm] {} (j2)
    %(i4) edge node [xshift = -0.3cm] {} (j3)
    %(i4) edge node [xshift = -0.3cm] {} (j4);
    
    \path[draw, line width = 0.25mm]
    %(i5) edge node [xshift = -0cm] {} (j4)
    (i1) edge node [xshift = 0.3cm] {} (j1)
    (i2) edge node [xshift = 0.3cm] {} (j1)
    (i3) edge node [xshift = 0.3cm] {} (j1)
    (i1) edge node [xshift = -0cm] {} (j3)
    (i2) edge node [xshift = -0cm] {} (j3)
    (i3) edge node [xshift = -0cm] {} (j3);
    %(i4) edge node [xshift = -0cm] {} (j4);
    
    \path[draw, line width = 0.25mm]
    %(i1) edge node [xshift = -0cm] {} (j2)
    (i2) edge node [xshift = -0cm] {} (j3);
    %(i3) edge node [xshift = -0cm] {} (j4);
    
\end{tikzpicture}} 
\caption{Choice of nodes}
\end{subfigure}
\begin{subfigure}[t]{0.45 \textwidth}
\centering
\resizebox{0.35\textwidth}{!}{
  \begin{tikzpicture}[-latex]
    \node[draw, circle, semithick, minimum size = 0.4cm] (i1) {$1$};
    \node[draw, circle, semithick, minimum size = 0.4cm] (i2) [below= 0.4cm of i1]  {$2$};
    \node[draw, circle, semithick, minimum size = 0.4cm] (i3) [below = 0.4cm of i2]  {$3$};
    \node[draw, circle, semithick, minimum size = 0.7cm] (j1) [right = 1.5cm of i1]  {a};
    \node[draw, circle, semithick, minimum size = 0.7cm] (j2) [below = 0.4cm of j1]  {b};
    \node[draw, circle, semithick, minimum size = 0.7cm] (j3) [below = 0.4cm of j2]  {c};
    \node[draw, circle, semithick, minimum size = 0.7cm] (j4) [below = 0.4cm of j3]  {d};
    %\node[draw, circle, fill = gray!15,minimum size = 0.15cm] (i4) [below = 0.4cm of i3]  {$i_4$};

    \path[draw, gray, line width = 0.05mm]
    (i1) edge node [xshift = -0.3cm] {} (j1)
    (i1) edge node [xshift = -0.3cm] {} (j2)
    (i1) edge node [xshift = -0.3cm] {} (j3)
    (i1) edge node [xshift = -0.3cm] {} (j4)
    (i2) edge node [xshift = -0.3cm] {} (j1)
    (i2) edge node [xshift = -0.3cm] {} (j2)
    (i2) edge node [xshift = -0.3cm] {} (j3)
    (i2) edge node [xshift = -0.3cm] {} (j4)
    (i3) edge node [xshift = -0.3cm] {} (j1)
    (i3) edge node [xshift = -0.3cm] {} (j2)
    (i3) edge node [xshift = -0.3cm] {} (j3)
    (i3) edge node [xshift = -0.3cm] {} (j4);
    %(i4) edge node [xshift = -0.3cm] {} (j1)
    %(i4) edge node [xshift = -0.3cm] {} (j2)
    %(i4) edge node [xshift = -0.3cm] {} (j3)
    %(i4) edge node [xshift = -0.3cm] {} (j4);
    
    \path[draw, line width = 0.25mm]
    %(i5) edge node [xshift = -0cm] {} (j4)
    (i1) edge node [xshift = 0.3cm] {} (j1)
    (i2) edge node [xshift = 0.3cm] {} (j2)
    (i3) edge node [xshift = -0cm] {} (j3);
    %(i4) edge node [xshift = -0cm] {} (j4);
    
    \path[draw, line width = 0.25mm]
    (i1) edge node [xshift = -0cm] {} (j2)
    (i2) edge node [xshift = -0cm] {} (j3)
    (i3) edge node [xshift = -0cm] {} (j4);
    
\end{tikzpicture}} 
\caption{Choice of links}
\end{subfigure}
\caption{Assignment problem where edge weights are unknown. In the first stage we can either select a set of nodes (as in (a)) or a set of links (as in (b)) for which those assignments become possible in the second stage when edge weights are known.}
\end{figure}

==> Tikz_Examples/Contingency_SP.tex <==
\begin{figure}[h]
\centering
\resizebox{0.4\textwidth}{!}{
  \begin{tikzpicture}[-{Latex[scale = 0.5]}]
    \node[draw, circle, scale=0.4] (1) {1};
    \node[draw, circle, scale=0.4] (2) [above right = 0.1cm and 0.3cm of 1]  {2};
    \node[draw, circle, scale=0.4] (3) [below right = 0.4cm and -0.1cm of 2]  {3};
    \node[draw, circle, scale=0.4] (5) [right = 1cm of 1]  {5};
    \node[draw, circle, scale=0.4] (6) [below left = 0.4cm and -0.1cm of 5]  {6};
    \node[draw, circle, scale=0.4] (4) [above = 0.4cm of 5]  {4};
    \node[draw, circle, scale=0.4] (9) [below right = 0.1cm and 0.5cm of 5]  {9};
    \node[draw, circle, scale=0.4] (8) [above right = 0.3cm and 0.1cm of 9]  {8};
    \node[draw, circle, scale=0.4] (7) [above right = 0.2cm and 0.3cm of 8]  {7};
    \node[draw, circle, scale=0.35] (10) [right = 0.4cm of 9]  {10};
    \node[draw, circle, scale=0.35] (11) [above right = 0.05cm and 0.4cm of 10]  {11};
    \node (13) [below right = 0.4cm and 0.5cm of 9]  {};
    %\node[draw, circle, fill = gray!15,minimum size = 0.15cm] (i4) [below = 0.4cm of i3]  {$i_4$};

    \path[draw, gray, line width = 0.01mm]
    (1) edge node [xshift = -0.3cm] {} (2)
    (1) edge node [xshift = -0.3cm] {} (3)
    (2) edge node [xshift = -0.3cm] {} (4)
    (2) edge node [xshift = -0.3cm] {} (5)
    (3) edge node [xshift = -0.3cm] {} (5)
    (3) edge node [xshift = -0.3cm] {} (6)
    (4) edge node [xshift = -0.3cm] {} (7)
    (4) edge node [xshift = -0.3cm] {} (8)
    (8) edge node [xshift = -0.3cm] {} (7)
    (5) edge node [xshift = -0.3cm] {} (8)
    (5) edge node [xshift = -0.3cm] {} (9)
    (6) edge node [xshift = -0.3cm] {} (9)
    (4) edge node [xshift = -0.3cm] {} (5)
    (9) edge node [xshift = -0.3cm] {} (10)
    (10) edge node [xshift = -0.3cm] {} (11)
    (8) edge node [xshift = -0.3cm] {} (10)
    (8) edge node [xshift = -0.3cm] {} (11)
    (7) edge node [xshift = -0.3cm] {} (11)
    (9) edge node [xshift = -0.3cm] {} (8)
    (6) edge node [xshift = -0.3cm] {} (5);
    
    \path[draw, red!60!white, line width = 0.2mm]
    %(1) edge node [xshift = -0.3cm] {} (2)
    %(2) edge node [xshift = -0.3cm] {} (4)
    %(4) edge node [xshift = -0.3cm] {} (7)
    %(7) edge node [xshift = -0.3cm] {} (11)
    (4) edge node [xshift = -0.3cm] {} (8)
    (8) edge node [xshift = -0.3cm] {} (7)
    (8) edge node [xshift = -0.3cm] {} (11);
    
    \path[draw, red!50!black, line width = 0.2mm]
    (1) edge node [xshift = -0.3cm] {} (2)
    (2) edge node [xshift = -0.3cm] {} (4)
    (4) edge node [xshift = -0.3cm] {} (7)
    (7) edge node [xshift = -0.3cm] {} (11);
    %(4) edge node [xshift = -0.3cm] {} (8)
    %(8) edge node [xshift = -0.3cm] {} (7)
    %(8) edge node [xshift = -0.3cm] {} (11);
    
    
\end{tikzpicture}} 
\caption{A subnetwork of paths between node (1) and (11).}\label{fig:routing}
\end{figure}

==> Tikz_Examples/First_Exs.tex <==
\begin{figure}[h]
\centering
\begin{subfigure}[t]{0.45 \textwidth}
\centering
\resizebox{0.8\textwidth}{!}{
  \begin{tikzpicture}[-{Latex[scale = 0.5]}]
    \node[draw, circle, scale=0.6] (1) {};
    \node[draw, circle, scale=0.6] (2) [above right = 0.1cm and 0.3cm of 1]  {};
    \node[draw, circle, scale=0.6] (3) [below right = 0.4cm and -0.1cm of 2]  {};
    \node[draw, circle, scale=0.6] (5) [right = 1cm of 1]  {};
    \node[draw, circle, scale=0.6] (6) [below left = 0.4cm and -0.1cm of 5]  {};
    \node[draw, circle, scale=0.6] (4) [above = 0.4cm of 5]  {};
    \node[draw, circle, scale=0.6] (9) [below right = 0.1cm and 0.5cm of 5]  {};
    \node[draw, circle, scale=0.6] (8) [above right = 0.3cm and 0.1cm of 9]  {};
    \node[draw, circle, scale=0.6] (7) [above right = 0.2cm and 0.3cm of 8]  {};
    \node[draw, circle, scale=0.6] (10) [right = 0.4cm of 9]  {};
    \node[draw, circle, scale=0.6] (11) [above right = 0.05cm and 0.4cm of 10]  {};
    \node (13) [below right = 0.4cm and 0.5cm of 9]  {};
    %\node[draw, circle, fill = gray!15,minimum size = 0.15cm] (i4) [below = 0.4cm of i3]  {$i_4$};

    \path[draw, gray, line width = 0.01mm]
    (1) edge node [xshift = -0.3cm] {} (2)
    (1) edge node [xshift = -0.3cm] {} (3)
    (2) edge node [xshift = -0.3cm] {} (4)
    (2) edge node [xshift = -0.3cm] {} (5)
    (3) edge node [xshift = -0.3cm] {} (5)
    (3) edge node [xshift = -0.3cm] {} (6)
    (4) edge node [xshift = -0.3cm] {} (7)
    (4) edge node [xshift = -0.3cm] {} (8)
    (8) edge node [xshift = -0.3cm] {} (7)
    (5) edge node [xshift = -0.3cm] {} (8)
    (5) edge node [xshift = -0.3cm] {} (9)
    (6) edge node [xshift = -0.3cm] {} (9)
    (4) edge node [xshift = -0.3cm] {} (5)
    (9) edge node [xshift = -0.3cm] {} (10)
    (10) edge node [xshift = -0.3cm] {} (11)
    (8) edge node [xshift = -0.3cm] {} (10)
    (8) edge node [xshift = -0.3cm] {} (11)
    (7) edge node [xshift = -0.3cm] {} (11)
    (9) edge node [xshift = -0.3cm] {} (8)
    (6) edge node [xshift = -0.3cm] {} (5);
    
    \path[draw, red!50!black, line width = 0.2mm]
    (1) edge node [xshift = -0.3cm] {} (2)
    (2) edge node [xshift = -0.3cm] {} (4)
    (4) edge node [xshift = -0.3cm] {} (7)
    (7) edge node [xshift = -0.3cm] {} (11)
    (4) edge node [xshift = -0.3cm] {} (8)
    (8) edge node [xshift = -0.3cm] {} (7)
    (8) edge node [xshift = -0.3cm] {} (11);
    
\end{tikzpicture}} 
\caption{Routing Problems}\label{fig:routing}
\end{subfigure}
\begin{subfigure}[t]{0.45 \textwidth}
\centering
\resizebox{0.35\textwidth}{!}{
  \begin{tikzpicture}[-latex]
    \node[draw, circle, semithick, minimum size = 0.4cm] (i1) {$1$};
    \node[draw, circle, semithick, minimum size = 0.4cm] (i2) [below= 0.4cm of i1]  {$2$};
    \node[draw, circle, semithick, minimum size = 0.4cm] (i3) [below = 0.4cm of i2]  {$3$};
    \node[draw, circle, very thick, red!50!black, minimum size = 0.7cm] (j1) [right = 1.5cm of i1]  {a};
    \node[draw, circle, semithick, minimum size = 0.7cm] (j2) [below = 0.4cm of j1]  {b};
    \node[draw, circle, very thick, red!50!black, minimum size = 0.7cm] (j3) [below = 0.4cm of j2]  {c};
    \node[draw, circle, semithick, minimum size = 0.7cm] (j4) [below = 0.4cm of j3]  {d};
    %\node[draw, circle, fill = gray!15,minimum size = 0.15cm] (i4) [below = 0.4cm of i3]  {$i_4$};

    \path[draw, gray, line width = 0.05mm]
    (i1) edge node [xshift = -0.3cm] {} (j1)
    (i1) edge node [xshift = -0.3cm] {} (j2)
    (i1) edge node [xshift = -0.3cm] {} (j3)
    (i1) edge node [xshift = -0.3cm] {} (j4)
    (i2) edge node [xshift = -0.3cm] {} (j1)
    (i2) edge node [xshift = -0.3cm] {} (j2)
    (i2) edge node [xshift = -0.3cm] {} (j3)
    (i2) edge node [xshift = -0.3cm] {} (j4)
    (i3) edge node [xshift = -0.3cm] {} (j1)
    (i3) edge node [xshift = -0.3cm] {} (j2)
    (i3) edge node [xshift = -0.3cm] {} (j3)
    (i3) edge node [xshift = -0.3cm] {} (j4);
    %(i4) edge node [xshift = -0.3cm] {} (j1)
    %(i4) edge node [xshift = -0.3cm] {} (j2)
    %(i4) edge node [xshift = -0.3cm] {} (j3)
    %(i4) edge node [xshift = -0.3cm] {} (j4);
    
    \path[draw, red!50!black, line width = 0.3mm]
    %(i5) edge node [xshift = -0cm] {} (j4)
    (i1) edge node [xshift = 0.3cm] {} (j1)
    (i2) edge node [xshift = 0.3cm] {} (j1)
    (i3) edge node [xshift = 0.3cm] {} (j1)
    (i1) edge node [xshift = -0cm] {} (j3)
    (i2) edge node [xshift = -0cm] {} (j3)
    (i3) edge node [xshift = -0cm] {} (j3)
    (i2) edge node [xshift = -0cm] {} (j3);
    
\end{tikzpicture}} 
\caption{Assignment Problems}\label{fig:assignment}
\end{subfigure}
\caption{Examples of problems where we want to minimize the sum of edge weights which are unknown in the first-stage. In Figure (a), we can identify a subset of links in the network for which we can construct a path once edge weights become known. In Figure (b), we can identify a subset of right-side nodes for which we can make an assignment of left-side nodes when edge weights become known. }
\end{figure}
